Segment-Level Diffusion: A Framework for Controllable Long-Form Generation with Diffusion Language Models

Diffusion models have shown promise in text generation, but often struggle with generating long, coherent, and contextually accurate text. Token-level diffusion doesn't model word-order dependencies explicitly and operates on short, fixed output windows, while passage-level diffusion struggles with learning robust representations for long-form text. To address these challenges, we propose Segment-Level Diffusion (SLD), a framework that enhances diffusion-based text generation through text segmentation, robust representation training with adversarial and contrastive learning, and improved latent-space guidance. By segmenting long-form outputs into multiple latent representations and decoding them with an autoregressive decoder, SLD simplifies diffusion predictions and improves scalability. Experiments on four datasets demonstrate that, when compared to other diffusion and autoregressive baselines SLD achieves competitive or superior fluency, coherence, and contextual compatibility in automatic and human evaluations.

==> src/03_preliminaries.tex <==
%THIS SECTION IS NO LONGER INCLUDED
\section{Preliminary}

%\neocomment{How about if I extract latent space diffusion and put it here, and move the diffusion model preliminaries to appendix?}
\subsection{Diffusion Model}

A diffusion model %is a generative framework that 
operates on latent variables $\mathbf{x} \in \mathbb{R}^d$ across $T$ time steps, modelled as a Markov chain \cite{sohl2015deep, ho2020denoising, song2020improved}. It consists of two processes: a backward process for inference and a forward process for training.

\rparagraph{Inference} The backward process generates a data point by iteratively removing noise from an initial noisy sample. Starting with a variable $\mathbf{x}_T \sim \mathcal{N}(\mathbf{x}_T; \mathbf{0}, \mathbf{I})$, the model with parameters $\theta$ predicts the  progressively de-noised variable $\mathbf{x}_{t-1}$ at each time step $t$ as follows:
\begin{equation}
    p(\mathbf{x}_{t-1} | \mathbf{x}_{t}; {\theta}) = \mathcal{N} \left( \mathbf{x}_{t-1}; \boldsymbol{\mu}(\mathbf{x}_{t}, t; {\theta}), \Sigma(\mathbf{x}_{t}, t; {\theta}) \right)
\end{equation}
where $\boldsymbol{\mu}(\mathbf{x}_{t}, t; {\theta})$ and $\Sigma(\mathbf{x}_{t}, t; {\theta})$ are the predicted mean and variance, respectively. The model iteratively refines the noisy sample $\mathbf{x}_T$ to recover $\mathbf{x}_0$, the de-noised datapoint. 

\rparagraph{Training}  
The model is trained by minimizing a regression loss to predict the noise added during the forward process. In the forward process, an observation $\mathbf{x}_0$ sampled from the data distribution $d(\mathbf{x})$ is gradually corrupted into Gaussian noise over $T$ time steps. This corruption is modelled as:
\begin{equation}
    q(\mathbf{x}_{t} | \mathbf{x}_{t-1}) = \mathcal{N} (\mathbf{x}_{t}; \sqrt{1-\beta_{t}}\mathbf{x}_{t-1}, \beta_{t}\mathbf{I}),
\end{equation}
where $\beta_t$ controls the variance of the added noise at each step. The objective is to minimize the distance between the predicted mean $\boldsymbol{\mu}(\mathbf{x}_t, t; \theta)$ and the true posterior mean $\hat{\boldsymbol{\mu}}(\mathbf{x}_t, \mathbf{x}_0)$, computed in closed form:
\begin{equation}
    \mathcal{L}(\theta) = \sum_{t=1}^T \underset{q(\mathbf{x}_{t} | \mathbf{x}_0)}{\mathbb{E}} \left\| \boldsymbol{\mu}(\mathbf{x}_{t}, t; {\theta}) - \hat{\boldsymbol{\mu}}(\mathbf{x}_{t}, \mathbf{x}_0) \right\|^2_2,
\end{equation}
where $\hat{\boldsymbol{\mu}}(\mathbf{x}_t, \mathbf{x}_0)$ is derived from the forward process. This loss trains the model to iteratively reverse the corruption applied during the forward process, enabling high-quality data generation in the backward process.
